Measuring Changes in Regional Network Traffic Due to COVID-19 Stay-at-Home Measures

During the 2020 pandemic caused by the COVID-19 virus, many countries implemented stay-at-home measures, which led to many businesses and schools moving from in-person to online mode of operation. We analyze sampled Netflow records at a medium-sized US Regional Optical Network to quantify the changes in the network traffic due to stay-at-home measures in that region. We find that human-driven traffic in the network decreases to around 70%, and mostly shifts to local ISPs, while VPN and online meeting traffic increases up to 5 times. We also find that networks adopt a variety of online meeting solutions and favor one but continue using a few others. We find that educational and government institutions experience large traffic changes, but aim to keep their productivity via increased online meetings. Some scientific traffic also reduces possibly leading to loss of research productivity. Businesses mostly lose their traffic and few show VPN or online meeting activity. Most network prefixes experience large loss of live addresses but a handful increase their liveness. We also find increased incidence of network attacks. Our findings can help plan network provisioning and management to prepare for future possible infection outbreaks and natural disasters.

==> individual_ip.tex <==
\section{Traffic changes of individual IP addresses}
\label{sec:individual}

We also track some individual IP addresses to analyse traffic changes from a user's perspective. 
Here, we only select IPs that are consistent and active, i.e., whose main purpose (e.g., Web server) does not change, and whose activity remains considerable during our observation period. 

We further classify the selected IPs into \emph{servers} and \emph{clients} by observing the distribution of their traffic over port numbers.
If the majority of traffic from an IP address are from a well-known server port towards a variety of high-numbered ports, we consider the IP address as a server IP. Otherwise it is a client IP. 

We filter out a set of qualified IP addresses, and then we select a handful of IPs with diverse purpose. 
Figures~\ref{fig:individual_ip} in Appendix illustrate the traffic volume changes of three server IPs and three client IPs  with Table~\ref{tab:ip_to_obse} summarizing their traffic changes.
The shaded areas show weekly traffic volume, and the lines show hourly traffic volume.
We also show more examples in Appendix~\ref{sec:more_ind_ip}.
We observe the following phenomena:
(1) The traffic changes of individual servers are very diverse, not necessarily following the application's overall direction of traffic change;
(2) Residential clients tend to generate more traffic after the transition, probably because the stay-at-home order focuses people's activities at home;
(3) The government and education clients tend to be less active after the transition; and
(4) The traffic transition of our select education clients happened before the traffic transition of our select government clients, due to the combined effect of both the stay-at-home measure and the school spring break.

\begin{table}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
        \textbf{IP} &\textbf{Nature}  & \multicolumn{2}{c}{\textbf{work-hours}} & \multicolumn{2}{c}{\textbf{rest-hours}} \\ \cline{3-6}
        & & change & aft/bef & change & aft/bef \\ \hline
        A & HTTPS server & $\downarrow$  & 59\% & $\downarrow$ & 62\% \\
        B & Unidata server & $\uparrow$  & 116\% & $\downarrow$ & 98\% \\
        C & Streaming server & $\uparrow$ & 1671\% & $\uparrow$ & 656\% \\
        D & Residential client & $\uparrow$  & 4318\% & $\uparrow$ & 45296\% \\
        E & Education client & $\downarrow$ & 11\% & $\downarrow$ & 14\% \\
        F & Government client & $\downarrow$  & 89\% & $\downarrow$ & 21\% \\
    \end{tabular}
    \caption{IP addresses to observe and their traffic changes}
    \label{tab:ip_to_obse}
\end{table}



